Efficient Deep Clustering of Human Activities and How to Improve Evaluation

There has been much recent research on human activity re\-cog\-ni\-tion (HAR), due to the proliferation of wearable sensors in watches and phones, and the advances of deep learning methods, which avoid the need to manually extract features from raw sensor signals. A significant disadvantage of deep learning applied to HAR is the need for manually labelled training data, which is especially difficult to obtain for HAR datasets. Progress is starting to be made in the unsupervised setting, in the form of deep HAR clustering models, which can assign labels to data without having been given any labels to train on, but there are problems with evaluating deep HAR clustering models, which makes assessing the field and devising new methods difficult. In this paper, we highlight several distinct problems with how deep HAR clustering models are evaluated, describing these problems in detail and conducting careful experiments to explicate the effect that they can have on results. We then discuss solutions to these problems, and suggest standard evaluation settings for future deep HAR clustering models. Additionally, we present a new deep clustering model for HAR. When tested under our proposed settings, our model performs better than (or on par with) existing models, while also being more efficient and better able to scale to more complex datasets by avoiding the need for an autoencoder.

==> scrap.tex <==
\begin{table}[]
\caption{Comparison of our clustering method and existing supervised methods: \protect\cite{dua2021multi} on PAMAP, UCI-Sm,  and WISDM-v1, \protect\cite{aljarrah2021human} on REALDISP, and \protect\cite{osia2020hybrid} on HHAR.\vspace*{1ex}}
\label{tab:supervised-comp}
\centering
\begin{tabular}{*{11}{|c}|}
\hline
% & \multicolumn{2}{c|}{HHAR} & \multicolumn{2}{c|}{PAMAP} & \multicolumn{2}{c|}{REALDISP} & \multicolumn{2}{c|}{UCI-Sm} & \multicolumn{1}{c|}{WISDM-v1} \\\hline
 & \multicolumn{2}{c|}{PAMAP} & \multicolumn{2}{c|}{UCI-Sm} & \multicolumn{2}{c|}{WISDM-v1} & \multicolumn{2}{c|}{REALDISP} & \multicolumn{1}{c|}{HHAR} \\\hline
 & ACC & F1 & ACC & F1 & ACC & F1 & ACC & F1 & ACC \\\hline\hline
	ours & 86.3 & 80.1 & 65.9 & 64.4 & 75.3 & 68.9 & 91.0 & 88.0 & 62.3 \\
\hline
	supervised & 95.3 & 95.2 & 96.2 & 96.2 & 97.2 & 97.2 & 99.8 & 99.8 & 94.2 \\
\hline
\end{tabular}
\end{table}


\begin{table}[!htb]
    \begin{minipage}{.45\linewidth}
 \caption{Comparison of our method with that of \cite{sheng2020unsupervised}. Ours performs better on both datasets and all metrics, with the difference being more significant on the more complex dataset, REALDISP.\vspace*{1ex}}
        \label{tab:sheng-comp}
        \centering
        \begin{tabular}{*{7}{|c}|}
        \hline
         & \multicolumn{3}{c|}{PAMAP} & \multicolumn{3}{c|}{REALDISP} \\\hline
         & ACC & ARI & NMI & ACC & ARI & NMI \\\hline\hline
        	ours & \textbf{86.3} & \textbf{88.4} & \textbf{81.4} & \textbf{91.0} & \textbf{95.2} & \textbf{88.9} \\
        \hline
        	S20 & 85.4 & 87.3 & 80.2 & 68.1 & 60.5 & 80.4 \\
        \hline
        \end{tabular}
    \end{minipage}%
    \hspace{14pt}
    \begin{minipage}{.45\linewidth}
       \centering
        \caption{Comparison of our method with that of \cite{ma2021unsupervised} on the HHAR dataset. We achieve a significantly higher NMI but a lower F1.\vspace*{1ex}} \label{tab:ma-comp}

        \begin{tabular}{*{3}{|c}|}
        \hline
         & \multicolumn{2}{c|}{HHAR} \\\hline
         & F1 & NMI \\\hline\hline
        	ours & \textbf{67.9} & 59.0 \\
        \hline
        	M21 & 55.0 & \textbf{65.9} \\
        \hline
        \end{tabular}     
    \end{minipage} 
\end{table}
\begin{table}[]
    \centering
        \caption{Comparison of our method with that of \cite{mcconville2021n2d} on the UCI-Sm dataset. We achieve a marginally higher NMI but a lower ACC.\vspace*{1ex}} \label{tab:n2d-comp}

        \begin{tabular}{*{3}{|c}|}
        \hline
         & \multicolumn{2}{c|}{HHAR} \\\hline
         & ACC & NMI \\\hline\hline
        	ours & \Uacc & \textbf{\Unmi} \\
        \hline
        	McC21 & \textbf{80.1} & 68.3 \\
        \hline
        \end{tabular}     
\end{table}

To show ACC formally, as an example
\begin{gather} \label{eq:cluster-accuracy}
    ACC = \max_{P \in S_K} \frac{1}{N}\sum_{i=1}^N \mathbbm{1}(\tilde{c}(x_i) = P(c(x_i)))\,, 
\end{gather}
where $K$ is the number of ground truth classes, $S_K$ is the permutation group on $K$ elements, $\tilde{c}(x)$ and $c(x)$ are, respectively, the assigned cluster label and the ground-truth class label for data point $x$, and $\mathbbm{1}$ is the indicator function. The permutation $P$ can be computed efficiently using the Hungarian algorithm. Macro-F1 is then computed using the standard definition, after applying the same permutation. 

\
